Quantifying the Impact of Stealthy BLE Spam & Flooding Attacks on IoT Environments

The energy-efficient design of the BLE protocol, emphasis on rapid, and userfriendly discovery, making it an ideal choice for IoMTs, specifically, military field medical systems, and battlefield wearable sensors. Especially in active conflict zones, when static medical facilities are vulnerable and often targeted, limiting their viability for sustained care delivery. This rapid deployment, and ease of management comes at the cost of expanded attack surface, i.e., BLE flooding attacks. During such attacks, adversaries flood advertisement channels with unauthorized connection or advertising requests to exhaust nearby device resources and disrupt legitimate communication, sometimes culminating in denial-of-service conditions. A first public proof-of-concept of such attacks, using a Raspberry Pi has since been adapted to commodity platforms (e.g., Flipper Zero, HackRF, Android), lowering the barrier to attack. In contested environments, such platforms are directly relevant to adversarial RF jamming and spoofing operations, where low-cost, portable devices can induce disproportionate disruption in dense wireless ecosystems. In this work, we develop a quantitative foundation for understanding the impact of such attacks and propose a practical deterrence strategy based on agility to raise the cost of such attacks.

==> dataset_compare_table2.tex <==
\begin{tabular}{
|>{\centering\arraybackslash}m{2.5cm}
|>{\centering\arraybackslash}m{3cm}
|>{\centering\arraybackslash}m{3cm}
|>{\centering\arraybackslash}m{3cm}
|>{\centering\arraybackslash}m{3cm}
|>{\centering\arraybackslash}m{3cm}
|>{\centering\arraybackslash}m{3cm}|
}
\hline
\textbf{Feature} & \textbf{BLEBeacon} & \textbf{Bluetack} & \textbf{SDR4IoT} & \textbf{University Dataset} & \textbf{CICIoMT} & \textbf{Our Dataset} \\
\hline
\textbf{Protocol} & BLE & BR/EDR + BLE & BLE + Zigbee & Bluetooth Classic & BLE, Wi-Fi, MQTT & BLE \\
\hline
\textbf{Data Type} & RSSI logs & Aggregated stats & Raw IQ + demodulated & Passive logs & Protocol event logs & Raw packet/ Advertisements \\
\hline
\textbf{BLE Layer} & Physical Layer & HCI + L2CAP layer (aggregated metrics) & Physical Layer & Baseband/Link layer (partial MAC + channel + SNR) & HCI & Link Layer \\
\hline
\textbf{Granularity} & 1 Hz & 100 ms window & Millisecond range (per frame start/end) & Sub-millisecond & Millisecond (ms) & Microsecond (\textmu s) \\
\hline 
\textbf{Attack Types}&	\ding{55}&	DoS, MITM, Bluesmack	& \ding{55} &	\ding{55} & DoS	& Advertisement Spam \\
\hline
\textbf{MAC Address Visibility} & \ding{55} & \ding{55} & \ding{55} & Partial (LAP only) & Limited & \checkmark \\
\hline
\textbf{Payload Inspection} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & Partial & \checkmark \\
\hline
\textbf{Advertising Channel Index} & \ding{55} & \ding{55} & via frequency & \checkmark & \ding{55} & \checkmark \\
\hline
\textbf{DoS Detection} & \ding{55} & \checkmark & \ding{55} & \ding{55} & \checkmark & \checkmark \\
\hline
\textbf{Beacon Spoofing Detection} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \checkmark \\
\hline
\textbf{Device Finger Printing} & \ding{55} & \ding{55} & \checkmark (RF based) & Limited & \checkmark & \checkmark \\
\hline
\textbf{Attack Attribution} & Low &	Moderate (role-based stats) &	High(RF fingerprinting) & Moderate (LAP+SNT+time) & Low & Moderate-High (Mac+timing)\\
\hline
 \textbf{Signature Attribution}	& Low & Moderate (Event patterns) &	Moderate(burst shape) &	Low–Moderate (recurrence scoring) & Moderate (GATT behavior types) & High (spam frequency + payload repeat)\\
\hline
\textbf{Use Case} & Proximity \& Presence Tracking & IDS for IoMT devices & RF fingerprinting \& Localization & Covert device detection during exams & Multi-Protocol IoMT security & Air-Interface spam/flood detection \\
\hline
\end{tabular}


==> dataset_compare_table3.tex <==
\begin{tabular}{
|>{\centering\arraybackslash}m{2.5cm}
|>{\centering\arraybackslash}m{3cm}
|>{\centering\arraybackslash}m{3cm}
|>{\centering\arraybackslash}m{3cm}
|>{\centering\arraybackslash}m{3cm}
|>{\centering\arraybackslash}m{3cm}
|>{\centering\arraybackslash}m{3cm}|
}
\hline
\textbf{Capability} & \textbf{Sikeridis et al.\cite{BLEbeacon}} & \textbf{Unal\cite{bluetack}} & \textbf{Duque et al.\cite{sdr4iot}} & \textbf{Bouaru et al.\cite{universitydataset}} & \textbf{Dadkhah et al.\cite{CICIoMT2024}} & \textbf{Our Behavioral Model} \\
\hline
\textbf{Attack Type Detection} & \ding{55} & DoS, MITM & \ding{55} & \ding{55} & DoS & DoS, Adv. Spam \\
\hline
\textbf{Profiling Support} & \ding{55} & Partial (role stats) & RF fingerprinting & Partial & \checkmark & \checkmark \\
\hline
\textbf{Behavioral Insight} & \ding{55} & Moderate & Moderate & Moderate & Low & High \\
\hline
\textbf{Attack Attribution} & Low &	Moderate (role-based stats) &	High(RF fingerprinting) & Moderate (LAP+SNT+time) & Low & Moderate-High (Mac+timing)\\
\hline
 \textbf{Signature Attribution}	& Low & Moderate (Event patterns) &	Moderate(burst shape) &	Low–Moderate (recurrence scoring) & Moderate (GATT behavior types) & High (spam frequency + payload repeat)\\
\hline
\textbf{Focus} & Tracking & IoMT IDS & RF Profiling & Device Detection & Multi-Protocol Logs & Behavior-based Threat Modeling\\

\hline
\end{tabular}



==> dataset_compare_table4.tex <==
\begin{tabular}{
>{\raggedright\arraybackslash}m{3.5cm}
>{\centering\arraybackslash}m{2.5cm}
>{\centering\arraybackslash}m{2.5cm}
>{\centering\arraybackslash}m{2.5cm}
>{\centering\arraybackslash}m{2.5cm}
>{\centering\arraybackslash}m{2.5cm}
>{\centering\arraybackslash}m{2.5cm}
}
\toprule

\textbf{Capability} & 
\textbf{Sikeridis et al.~\cite{BLEbeacon}} & \textbf{Unal~\cite{bluetack}} & \textbf{Duque et al.~\cite{sdr4iot}} & \textbf{Bouaru et al.~\cite{universitydataset}} & \textbf{Dadkhah et al.~\cite{CICIoMT2024}} & \textbf{Our Behavioral Model} \\
\midrule

\textbf{Classification} & Dataset \newline (BLE) & Dataset \newline(Bluetooth 4.0+) & Dataset \newline(BLE \& Zigbee) & Dataset \newline(Bluetooth)& Dataset \newline(BLE) & Probabilistic Modeling \\

\textbf{Possible Use Case} & User Mobility & Limited Intrusion Detection & Device Fingerprinting, Localization & User Localization & Intrusion Detection & Modeling \\

\textbf{Attack Type} & None & DoS, MITM & None & None & DoS & DoS, Adaptive Spam \\

\textbf{Attacker Profiling} & \rule{0pt}{1.9em} \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \checkmark \\

\textbf{Behavioral Dynamics} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \checkmark \\

\textbf{Agent Agility} & \rule{0pt}{1.9em} \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \checkmark \\

\textbf{Impact Estimation} & \rule{0pt}{1.9em} \ding{55} & \ding{55} & \ding{55} & \ding{55} & Limited & \checkmark \\

\textbf{Model Validation} & \rule{0pt}{1.9em} \ding{55} & \ding{55}& \ding{55} & \ding{55} & \ding{55} & Moderate--High \\

\textbf{Engagement Dynamics} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & Limited (Static) & \checkmark \\

\textbf{Focus }& Tracking & IoMT IDS & RF Fingerprinting & Device Localization & IoMT IDS & Behavior-based Threat Modeling \\

\bottomrule
\end{tabular}

\iffalse
\begin{tabular}{
|>{\centering\arraybackslash}m{3.5cm}
|>{\centering\arraybackslash}m{2.5cm}
|>{\centering\arraybackslash}m{2.5cm}
|>{\centering\arraybackslash}m{2.5cm}
|>{\centering\arraybackslash}m{2.5cm}
|>{\centering\arraybackslash}m{2.5cm}
|>{\centering\arraybackslash}m{2.5cm}|
}
\hline
\textbf{Capability} & \textbf{Sikeridis et al.~\cite{BLEbeacon}} & \textbf{Unal~\cite{bluetack}} & \textbf{Duque et al.~\cite{sdr4iot}} & \textbf{Bouaru et al.~\cite{universitydataset}} & \textbf{Dadkhah et al.~\cite{CICIoMT2024}} & \textbf{Our Behavioral Model} \\
\hline
\textbf{Attack Type} & None & DoS, MITM & None & None & DoS & DoS, Adaptive Spam\\
\hline
\textbf{Attacker Profiling} & \ding{55} & Partial & Partial (device RF profiles) & Partial (device usage patterns) & \ding{55} & \checkmark \\
\hline
\textbf{Behavioral Dynamics} & Partial (adv. intervals) & Partial (attack traffic patterns) & \ding{55} & \ding{55} & Partial (DoS timing)  & \checkmark \\
\hline
\textbf{Agent Agility} & \ding{55} \rule{0pt}{1.9em} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \checkmark \\
\hline
\textbf{Impact Estimation} & \rule{0pt}{1.9em} \ding{55} & Limited & \ding{55} & \ding{55} & Limited & \checkmark \\
\hline
\textbf{Model Validation}& Low & Moderate (role-based) & High (RF fingerprinting) & Moderate & Low & Moderate--High \\
\hline
\textbf{Engagement Dynamics} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & Partial (multi-protocol context) & \checkmark \\
\hline
\textbf{Focus} & Tracking & IoMT IDS & RF Profiling & Device Detection & Multi-Protocol Logs & Behavior-based Threat Modeling\\
\hline
\end{tabular}
\fi





==> table-2.2.tex <==
% Requires: \usepackage{array,booktabs,pifont}
\begin{tabular}{
>{\raggedright\arraybackslash}m{3 cm}
*{7}{>{\centering\arraybackslash}m{2.8cm}}
}
\toprule
\textbf{Capability} &
\textbf{Karim~\textit{et al.}~\cite{BLEdiff}} &
\textbf{Zhang~\textit{et al.}~\cite{BLESS}} &
\textbf{Che~\textit{et al.}~\cite{BlueSwat}} &
\textbf{Yaseen~\textit{et al.}~\cite{Marc}} &
\textbf{Wu~\textit{et al.}~\cite{FormalModel}} &
\textbf{Ray~\textit{et al.}~\cite{securityTestingFramework}} &
\textbf{Our Behavioral Model}
\\
\midrule

\textbf{Classification} &
Framework &
Framework &
Framework &
Framework &
Framework &
Framework &
Probabilistic Modeling
\\

\textbf{Possible Use Case} &
Compliance testing; deviation/attack discovery &
Audit BLE apps for encryption \& authentication &
Session-based Monitoring &
Anomaly Detection &
Protocol Verification &
Security Testing &
Modeling
\\

\textbf{Attack Type} &
DoS/Crash/Security bypass (via noncompliance) &
\ding{55} &
Session- \& packet-based attacks &
MITM, cloned-node &
Property Violations &
MITM, DoS (flood), fuzzing &
DoS, Adaptive Spam
\\

\textbf{Attacker Profiling} &
\ding{55} &
\ding{55} &
Partial (state-path patterns) &
\ding{55} &
\ding{55} &
\ding{55} &
\checkmark
\\

\textbf{Behavioral Dynamics} &
\ding{55} &
\ding{55} &
Partial (session FSM; sequential context) &
\ding{55} &
\ding{55} &
Partial (adv/conn-phase tests) &
\checkmark
\\

\textbf{Agent Agility} &
\ding{55} &
\ding{55} &
\ding{55}\,(policies updatable, not adaptive agents) &
\ding{55} &
\ding{55} &
\ding{55} &
\checkmark
\\

\textbf{Impact Estimation} &
\ding{55} &
Limited (insecure-app prevalence) &
\ding{55} &
\ding{55} &
\ding{55} &
\ding{55} &
\checkmark
\\

\textbf{Model Validation} &
High: Protocol-based &
High: Application Testing &
High &
Moderate &
High &
Low &
Moderate--High
\\

\textbf{Engagement Dynamics} &
\ding{55} &
\ding{55} &
\ding{55} \newline (no multi-actor) &
\ding{55} &
\ding{55} &
\ding{55} &
\checkmark
\\

\textbf{Focus} &
Implementation noncompliance \& exploit discovery &
App Security Scanning &
Runtime mitigation, State-aware defense &
Threshold based detection &
Spec verification across BC/BLE/Mesh &
BLE attack test suite &
Behavior-based Threat Modeling
\\

\bottomrule
\end{tabular}



\iffalse
\begin{tabular}{
>{\raggedright\arraybackslash}m{3.6cm}
*{6}{>{\centering\arraybackslash}m{2.9cm}}
}
\toprule
\textbf{Capability} &
\textbf{BLEDi\!ff} &
\textbf{BLESS} &
\textbf{BlueSWAT} &
\textbf{MARC} &
\textbf{Formal Model-Driven Discovery} &
\textbf{BLE Sec. Testing Framework}
\\
\midrule

\textbf{Classification} &
Framework &
Framework &
Framework &
Framework &
Framework &
Framework
\\

\textbf{Possible Use Case} &
Compliance testing; deviation/attack discovery &
Audit BLE apps for encryption \& authentication &
Session-based Monitoring &
Anomaly Detection &
Protocol Verification & Security Testing
\\

\textbf{Attack Type} &
DoS/Crash/Security bypass (via noncompliance) &
\ding{55} &
Session- \& packet-based attacks &
MITM, cloned-node &
Property Violations &
MITM, DoS (flood), fuzzing
\\

\textbf{Attacker Profiling} &
\ding{55} &
\ding{55} &
Partial (state-path patterns) &
\ding{55} &
\ding{55} &
\ding{55}
\\

\textbf{Behavioral Dynamics} &
\ding{55} &
\ding{55} &
Partial (session FSM; sequential context) &
\ding{55} &
\ding{55} &
Partial (adv/conn-phase tests)
\\

\textbf{Agent Agility} &
\ding{55} & \ding{55} & \ding{55}\,(policies updatable, not adaptive agents) & \ding{55} & \ding{55} & \ding{55}
\\

\textbf{Impact Estimation} &
\ding{55} &
Limited (insecure-app prevalence) &
\ding{55} &
\ding{55} &
\ding{55} &
\ding{55}
\\

\textbf{Model Validation} &
High: Protocol-based &
High: Application Testing &
High &
Moderate  &
High  &
Low 
\\

\textbf{Engagement Dynamics} &
\ding{55} &
\ding{55} &
\ding{55} \newline (no multi-actor)&
\ding{55} &
\ding{55} &
\ding{55}
\\

\textbf{Focus} &
Implementation noncompliance \& exploit discovery &
App Security Scanning &
Runtime mitigation, State-aware defense &
Threshold based detection &
Spec verification across BC/BLE/Mesh &
BLE attack test suite
\\

\bottomrule
\end{tabular}\fi

